MemTrace: Tracing and Attributing Errors in Large Language Model Memory Systems

Memory is essential for enabling large language models to support long-horizon reasoning, yet existing memory systems remain unreliable and difficult to debug. Tracing memory's dynamic evolution is crucial to understand how information is synthesized, propagated, or corrupted over time. In this work, we study the new problem of error tracing and attribution in LLM memory systems. We propose a novel framework that transforms memory pipelines into executable memory evolution graphs, enabling fine-grained tracing of operational information flow. We then construct MemTraceBench, a benchmark collected from representative memory systems such as Long-Context, RAG, Mem0, and EverMemOS, to systematically study memory failure modes. We further introduce an automatic attribution method that iteratively traces operation subgraphs to pinpoint the root cause of any failed case. Our analysis reveals that memory failures are systematic, stemming from operation-level issues like information loss and retrieval misalignment. Crucially, we leverage these fine-grained attribution signals to guide downstream prompt optimization, establishing a closed-loop system that automatically corrects faults and boosts end-task performance by up to 7.62 percentage points. Code has ben released at https://github.com/zjunlp/MemTrace.

==> section/2.draft.tex <==
\section{Problem Formulation}
\label{sec:problem_formulation}

In this section, we formally define the failure attribution problem for stateful agentic systems. Unlike previous works \cite{DBLP:conf/icml/ZhangY0LHZL0W0W25, Zhang2025AgenTracerWI, Wang2026FromFL}. For instance, in $\texttt{Mem0}^{\tiny g}$ \cite{Chhikara2025Mem0BP} that rely on a strictly sequential, turn-based protocol, modern stateful agents (e.g., systems equipped with non-parametric memory systems) involve complex, asynchronous, and non-linear information flows, an fact extraction process and an entity extraction process may occur concurrently, or an update action may implicitly depend on an existing memory unit created earlier. To accommodate such asynchronous and concurrent dependencies, we model the system's execution trace as a graph and formulate the failure attribution problem as finding the earliest and minimal causal cut-set of faulty operations. 

\subsection{Execution Graph and Trajectory}

Specifically, we conceptualize the agentic system's execution trace as a Directed Acyclic Bipartite Graph (DABG) $\mathcal{G} = (\mathcal{V}, \mathcal{O}, \mathcal{E})$. Here, $\mathcal{V}$ denotes the set of variables, representing tangible artifacts generated during system execution such as raw messages, memory units, and prompts. $\mathcal{O}$ represents the set of operations, such as LLM inference steps, tool invocations or parsing functions. The directed edges $\mathcal{E}$ capture the information flow, where each operation $o \in \mathcal{O}$ receives a subset of variables as inputs, denoted as $\text{In}(o) \subset \mathcal{V}$, and produces new variables as outputs, denoted as $\text{Out}(o) \subset \mathcal{V}$. A complete system execution yields a dynamic trajectory $\tau$, which is a specific instantiation of $\mathcal{G}$. We define a binary indicator $Z(\tau) \in \{0, 1\}$ to denote the final outcome of the trajectory, where $Z(\tau) = 1$ indicates a task failure and $Z(\tau) = 0$ indicates a success. 

\subsection{Decisive Error Set Objective}

Suppose an original trajectory fails, resulting in $Z(\tau) = 1$. Our objective is to directly identify the \textbf{earliest} and \textbf{minimal} causal cut-set of faulty operations, which we formally term the \textbf{Decisive Error Set}. To construct this definition, let $O_c \subseteq \mathcal{O}$ be a candidate set of operations. We determine that $O_c$ qualifies as a valid causal cut-set if it strictly satisfies three prerequisites. First, every individual operation within $O_c$ must be definitively faulty in its execution. Second, all operations within its strictly upstream ancestor set, denoted as $\text{Anc}(O_c)$, must be functionally correct. Third, we apply a graph-based counterfactual intervention: we construct a modified trajectory $\tau^{(O_c, *)}$ by replacing the faulty output variables of $O_c$ with their correct counterparts, while assuming an ideal execution policy for all strictly downstream descendant operations in $\text{Desc}(O_c)$. A candidate set is deemed causally sufficient if this specific intervention successfully rescues the failed trajectory, yielding $Z(\tau^{(O_c, *)}) = 0$.

We denote the complete space of candidate sets that satisfy the aforementioned conditions as $\mathcal{C}(\tau)$. The decisive error set $\mathcal{O}^*$ is then defined by imposing a strict minimality constraint on this feasible space. Specifically, the minimal property dictates that removing any arbitrary operation from $\mathcal{O}^*$ would break the causal sufficiency (i.e., the trajectory would fail again), meaning no strictly smaller subset of operations can achieve the successful outcome. Consequently, the failure attribution objective is expressed mathematically as:
\begin{equation}
\mathcal{O}^* \in \left\{ O_c \in \mathcal{C}(\tau) \mid \nexists O' \in \mathcal{C}(\tau): O' \subset O_c \right\}
\end{equation}
By optimizing this formulation, the attribution problem is reduced to locating a minimal topological frontier of errors that fundamentally disrupted the execution graph.

==> section/formula.tex <==
% \onecolumn
% \[
% \theta_c = \frac{|f_1| + |v| + \sum_{(q, a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(a_t \mid q, a_{<t}, f_1)]}
% {|f_0| + L_c \log_2 m}.
% \]

% \begin{equation}
% \begin{aligned}
% \mathrm{Preference}(c) \triangleq 
% \mathbb{E}_{(q,a)\in\mathcal{D}_c} \left[ \frac{1}{T(a)}
%     \sum_{t=1}^{T(a)} 
%     \log P_v(a_t \mid q, a_{<t}, f_1) 
% \right]
% \end{aligned}
% \label{eq:preference_def}
% \end{equation}

% {\small
% \begin{equation}
% \mathrm{Preference}
% = 
% \frac{
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{c}}
%     \sum_{t=1}^{T(a)}
%     \big[\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{c}} T(a)
% }.
% \end{equation}
% }

% {\small
% \begin{equation}
% \mathrm{Total}
% = 
% \frac{
%     |f_1| + |v| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}\cup{D}_{pos}}
%     \sum_{t=1}^{T(a)}
%     \big[-\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     |f_0| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}\cup{D}_{pos}} T(a) \log_2 m
% }.
% \label{eq:sft_compression_score}
% \end{equation}
% }

% {\small
% \begin{equation}
% \mathrm{Margin}
% = 
% \frac{
%     |f_1| + |v| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}}
%     \sum_{t=1}^{T(a)}
%     \big[-\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     |f_0| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}} T(a) \log_2 m
% }
% -
% \frac{
%     |f_1| + |v| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{pos}}
%     \sum_{t=1}^{T(a)}
%     \big[-\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     |f_0| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{pos}} T(a) \log_2 m
% }.
% \label{eq:sft_compression_score}
% \end{equation}
% }

% {\small
% \begin{equation}
% \mathrm{\theta_{neg}}
% = 
% \frac{
%     |f_1| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}}
%     \sum_{t=1}^{T(a)}
%     \big[-\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     |f_0| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}} T(a) \log_2 m
% }
% , 
% \mathrm{\theta_{pos}}
% = 
% \frac{
%     |f_1| + 
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{pos}}
%     \sum_{t=1}^{T(a)}
%     \big[-\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     |f_0| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{pos}} T(a) \log_2 m
% }.
% \label{eq:sft_compression_score}
% \end{equation}
% }

% \begin{CJK}{UTF8}{gbsn}
% 预训练压缩率 $\theta_c$ 定义为：
% \end{CJK}
% \[
% \theta_{pre} = \frac{|f_1| + \sum_{x \in \mathcal{D}_{pre}} \sum_{t=1}^{T(x)} [-\log_2 P(x_t \mid  x_{<t}, f_1)]}
% {|f_0| + \sum_{x \in \mathcal{D}_{pre}} T(x) \log_2 m}.
% \]

% % \begin{CJK}{UTF8}{gbsn}
% % 后训练压缩率 $\theta_c$ 定义为：
% % \end{CJK}
% % \[
% % \theta_{post} = \alpha\theta_{pre} + \beta\frac{|f_1'| + |v| + \sum_{(q, a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(a_t \mid q, a_{<t}, f_1)]}
% % {\sum_{(q,a) \in \mathcal{D}_{c}} T(a) \log_2 m}
% % \]

% \begin{CJK}{UTF8}{gbsn}
% 后训练压缩率 $\theta_c$ 定义1为：
% \end{CJK}
% \[
% \theta_{post} = \frac{|f_1| + \sum_{x \in \mathcal{D}_{pre}} \sum_{t=1}^{T(x)} [-\log_2 P(x_t \mid  x_{<t}, f_1)]+|f_1'| + |v| + \sum_{(q, a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(a_t \mid q, a_{<t}, f_1’)]}
% {|f_0| + \sum_{x \in \mathcal{D}_{pre}} T(x) \log_2 m+\sum_{(q,a) \in \mathcal{D}_{c}} T(a) \log_2 m}
% \]

% \begin{CJK}{UTF8}{gbsn}
% 压缩率可以只考虑数据压缩不考虑其他协议吗？：
% \end{CJK}
% \[
% \theta_{post} = \frac{\sum_{(q, a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(a_t \mid q, a_{<t})]}
% {\sum_{(q,a) \in \mathcal{D}_{c}} T(a) \log_2 m}
% \]

% \twocolumn

% \begin{CJK}{UTF8}{gbsn}
% \section{偏好的定义}

% 在基于概率的生成式语言模型中，\textbf{偏好}（Preference）指的是模型在给定输入条件下，对某一类回答的\emph{生成倾向}。这种倾向可由模型在生成完整回答时的平均 token 对数概率进行刻画，以消除不同长度的影响。概念上，偏好反映了模型概率分布对该类型回答的整体支持程度。

% 设：
% \begin{itemize}
%     \item $\mathcal{D}_c = \{(q, a)\}$ 表示类别为 $c$ 的语料集合，其中 $c\in\mathcal{C}$ 为回答类型，例如正类$(+)$或负类$(-)$。
%     \item $T(a)$ 表示回答 $a$ 的 token 总长度。
%     \item $a_{<t}$ 表示回答中第 $t$ 个 token 之前的所有 token。
%     \item $P_v(a_t \mid q, a_{<t}, f_1)$ 表示模型（参数 $v$）在给定问题 $q$、已生成 token $a_{<t}$ 及附加条件 $f_1$ 的情况下，生成 $a_t$ 的条件概率。
% \end{itemize}

% 在此设定下，类别 $c$ 的\textbf{偏好}定义为：
% \begin{equation}
% \begin{aligned}
% &\mathrm{Preference}(c) \triangleq \\
% &\mathbb{E}_{(q,a)\in\mathcal{D}_c} \left[ \frac{1}{T(a)}
%     \sum_{t=1}^{T(a)} 
%     \log P_v(a_t \mid q, a_{<t}, f_1) 
% \right]
% \end{aligned}
% \label{eq:preference_def}
% \end{equation}

% 该定义的含义为：
% \begin{enumerate}
%     \item 内层求和：计算该类回答每个 token 的条件概率的对数，并求平均，以得到回答整体的平均 token 概率（log 空间）。
%     \item 外层期望：对类别 $c$ 的所有样本取平均，得到模型在该类回答上的平均 log-likelihood。
% \end{enumerate}

% 基于上述定义，不同类别的\emph{偏好差距}可表示为：
% \begin{equation}
% \mathrm{Gap}(c_1, c_2) = \mathrm{Preference}(c_1) - \mathrm{Preference}(c_2),
% \label{eq:preference_gap}
% \end{equation}
% 该差值刻画了模型在两类回答上的倾向性差异。
% 当 $\mathrm{Gap}(+,-) > 0$ 时，模型更偏向类别 $+$（如积极回答），反之则偏向类别 $-$（如消极回答）。
% \end{CJK}

% \begin{CJK}{UTF8}{gbsn}
% \subsection{Preference 与 $\theta$ 的关系}

% 设：
% \begin{itemize}
%     \item 类别 $c \in \{\text{pos}, \text{neg}\}$；
%     \item $L_c = \sum_{(q,a) \in \mathcal{D}_c} T(a)$ 为类别 $c$ 的总 token 数；
%     \item $m$ 为词表大小；
%     \item $|f_0|, |f_1|$ 为常数项。
% \end{itemize}

% 偏好的定义为：
% \[
% \mathrm{Preference}(c) = 
% \frac{\sum_{(q,a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} \log_2 P_v(a_t \mid q, a_{<t}, f_1)}{L_c}.
% \]

% 原始压缩评分 $\theta_c$ 定义为：
% \[
% \theta_c = \frac{|f_1| + |v| + \sum_{(q, a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(a_t \mid q, a_{<t}, f_1)]}
% {|f_0| + L_c \log_2 m}.
% \]

% 注意到：
% \[
% \sum_{(q,a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(\ldots)] = -\,L_c \cdot \mathrm{Preference}(c),
% \]
% 因此有以下转换关系：

% \paragraph{用 Preference 表示 $\theta$}
% \begin{align}
% \theta_c &= \frac{|f_1| + |v| - L_c \cdot \mathrm{Preference}(c)}{|f_0| + L_c \log_2 m}, \label{eq:theta_from_pref_exact} \\
% \theta_c &\approx -\,\frac{\mathrm{Preference}(c)}{\log_2 m} \quad \text{(近似，忽略常数项)}. \label{eq:theta_from_pref_approx}
% \end{align}

% \paragraph{用 $\theta$ 表示 Preference}
% \begin{align}
% \mathrm{Preference}(c) &= \frac{|f_1| + |v| - \theta_c\left(|f_0| + L_c \log_2 m\right)}{L_c}, \label{eq:pref_from_theta_exact} \\
% \mathrm{Preference}(c) &\approx -\,\theta_c \,\log_2 m \quad \text{(近似，忽略常数项)}. \label{eq:pref_from_theta_approx}
% \end{align}

% 上述精确关系式(\ref{eq:theta_from_pref_exact})-(\ref{eq:pref_from_theta_exact})为一一对应的转换公式，而近似关系式(\ref{eq:theta_from_pref_approx})-(\ref{eq:pref_from_theta_approx})在忽略常数项、样本长度分布相对均匀的情况下成立。


% 此时，偏好差距可以使用压缩率表示为：
% \begin{equation}
% \begin{split}
% \mathrm{Gap}(c_1, c_2) &= \frac{|f_1| + |v| - \theta_{c_1}\left(|f_0| + L_{c_1} \log_2 m\right)}{L_{c_1}} \\
% &- \frac{|f_1| + |v| - \theta_{c_2}\left(|f_0| + L_{c_2} \log_2 m\right)} {L_{c_2}}, \\
% \mathrm{Gap}(c_1, c_2) 
% &\approx \left(\theta_{c_2} - \theta_{c_1}\right)\log_2 m.
% \end{split}
% \label{eq:gap_theta}
% \end{equation}

% \end{CJK}

